A practical guide to light-sheet microscopy for nanoscale imaging: Looking beyond the cell

We present a comprehensive guide to light-sheet microscopy (LSM) to assist scientists in navigating the practical implementation of this microscopy technique. Emphasizing the applicability of LSM to image both static microscale and nanoscale features, as well as diffusion dynamics, we present the fundamental concepts of microscopy, progressing through beam profile considerations, to image reconstruction. We outline key practical decisions in constructing a home-built system and provide insight into the alignment and calibration processes. We briefly discuss the conditions necessary for constructing a continuous 3D image and introduce our home-built code for data analysis. By providing this guide, we aim to alleviate the challenges associated with designing and constructing LSM systems and offer scientists new to LSM a valuable resource in navigating this complex field.

==> latexmkrc.tex <==
$ENV{'TEXINPUTS'}='./tex/:' . $ENV{'TEXINPUTS'}; 
$ENV{'BSTINPUTS'}='./bst/:' . $ENV{'BSTINPUTS'};
